Entropy numbers of finite dimensional mixed-norm balls and function space embeddings with small mixed smoothness

We study the embedding $\text{id}: \ell_p^b(\ell_q^d) \to \ell_r^b(\ell_u^d)$ and prove matching bounds for the entropy numbers $e_k(\text{id})$ provided that $0<p<r\leq \infty$ and $0<q\leq u\leq \infty$. Based on this finding, we establish optimal dimension-free asymptotic rates for the entropy numbers of embeddings of Besov and Triebel-Lizorkin spaces of small dominating mixed smoothness which settles an open question in the literature. Both results rely on a novel covering construction recently found by Edmunds and Netrusov.

==> Entropy.tex <==
\section{Results of Edmunds/Netrusov simplified}

Let $\upsilon: \R_+ \to \{2^k: k \in \N_0\}$ be given by $\log_2(\upsilon(x)) = \max\{0,\lceil \log_2(x) \rceil \}$. If $x \in [0,1]^b$, where $b \in \N$, we let $\upsilon(x) := b^{-1} (\upsilon(bx_1),\dots, \upsilon(bx_b))$.

\begin{lemma}[Simplification of EdNe, Lemma 2.2]
Let $\Gamma(b) = \upsilon(S(b))$, where $S(b) = \{ x \in [0,1]^b: \sum_{i=1}^b x_i \leq 1\}$ is the $b$-dimensional simplex. Then $\sharp \Gamma(b) \leq 2^{3b}$.
\end{lemma}

\begin{proof}
Given $x \in S(b)$, let $v = \upsilon(x)$. We clearly have $\sum_{i=1}^b v_i \leq 2$ and $b v_i \in \N$ for all $i=1,\dots,b$. Further
\[
 \sharp \{ i \in 1:b :  v_i \geq t \} \leq 2/t.
\]
Now let
\begin{align*}
 A(v,k) &:= \{  i \in 1:b: v_i = 2^k/b  \}, \quad k \in \N_0\\
 B(v,k) &:= \{ i \in 1:b: v_i \geq 2^k/b \}.
\end{align*}
Clearly, $\sharp A(v,k) \leq \sharp B(v,k) \leq \min \{b, b2^{1-k}\}$. Varying over all elements in the simplex, $A(v,0)$ can be any of the $2^b$ subsets of $1:b$. Fixing $A(v,0)$, there are at most $2^b$ possibilities for $A(v,1)$. Fixing $A(v,0)$ up to $A(v,k-1)$, there are at most $2^{b2^{1-k}}$ possibilities for $A(v,k)$. Hence, in total the set $\Gamma(b)$ may contain at most
\[ 
 2^b \cdot 2^b \cdot \sum_{k=2}^\infty 2^{b2^{k-1}} = 2^{3b}
\]
many elements.
\end{proof}

\section{Covering and packing constructions for mixed sequence spaces}\label{sec:coverings_and_packings}

We organize this section as follows. First, in Section \ref{sec:entropy_matching_bounds}, we present those parameter constellations where we are able to obtain matching bounds. Subsequently, we present a number of covering and packing constructions upon which the findings in Section \ref{sec:entropy_matching_bounds} rely. Some of the results are formulated in greater generality than needed in Section \ref{sec:entropy_matching_bounds}, which might be of independent interest. Section \ref{sec:entropy:p=r} deals with constructions that exploit the known bavior of $e_n(B_{\ell_q^d}, \ell_u^d)$. Section \ref{sec:entropy:q=u} is devoted to a generalization of the well-known Edmunds-Triebel covering.
\[ 
 e_n(B_{\ell_p^b(X)}, \ell_r^b(Y)).
\]

We devote our attention at first to the special case $r=\infty$.

In turns out that the behavior of these entropy numbers is completely attributed to the behavior of the entropy numbers $e_{n/b}(B_X,Y)$. In case that $p=\infty$, the simple structure of the mixed spaces makes it straightforward to see this. By taking the $b$-fold Cartesian product, a maximal $\varepsilon$-packing of $B_X$ in $Y$ with cardinality $m$ leads to a $\varepsilon$-packing of $B_{\ell_\infty^b(X)}$ in $\ell_\infty^b(Y)$ with cardinality $m^b$. Likewise, the $b$-fold Cartesian product of a minimal $\varepsilon$-covering of $B_X$ in $Y$ with cardinality $m$ provides us with a $\varepsilon$-covering of $B_{\ell_\infty^b(X)}$ in $\ell_\infty^b(Y)$ with cardinality $m^b$. This immediately translates into the following bounds on entropy numbers.

\begin{lemma}
Let $X$ and $Y$ be (quasi-)Banach spaces. For any $\varepsilon > 0$, we have
\begin{align*}
 \mathcal P(B_{\ell_\infty^b(X)}, \|\cdot\|_{\ell_\infty^b(Y)}, \varepsilon) &\geq \big( \mathcal P(B_X, \|\cdot\|_Y, \varepsilon) \big)^b\\
 \mathcal N(B_{\ell_\infty^b(X)}, \|\cdot\|_{\ell_\infty^b(Y)}, \varepsilon) &\leq \big( \mathcal N(B_X, \|\cdot\|_Y, \varepsilon) \big)^b
\end{align*}
\end{lemma}

%\begin{proof}
%%We prove
%%\[ 
%% 1/2 \, e_{\lceil n/b+1 \rceil}(\id: \ell_q^d \to \ell_u^d) \leq e_n(\id: \ell_\infty^b(\ell_q^d) \to \ell_\infty^b(\ell_u^d)) \leq e_{\lfloor (n-1)/b+1 \rfloor}(\id: \ell_q^d \to \ell_u^d).
%%\]
%\textbf{Lower bound:} Let $m = 2^{\lceil n/b +1 \rceil - 1}$. Let $\varepsilon > 0$ be such that the maximal $\varepsilon$-packing $P$ of $B_{\ell_q^d}$ in $\ell_u^d$ has $\card(P) \leq m$. Clearly $\varepsilon \geq \varepsilon_{\lceil n/b +1 \rceil}(\id: \ell_q^d \to \ell_u^d)$. The Cartesian product $P^b$ of the maximal packing $P$ is contained in $B_{\ell_\infty^b(\ell_q^d)}$ and for any $x,y \in P^b$ with $x \neq y$ we have $\|x-y\|_{\infty,u} > \varepsilon$. Hence $P^b$ is a $\varepsilon$-packing with cardinality $\card(\mathcal P^b) = m^b$. For $\delta = e_n(\id: \ell_\infty^b(\ell_q^d) \to \ell_\infty^b(\ell_u^d))$, consider now a minimal $\delta$-covering K of $B_{\ell_\infty^b(\ell_q^d)}$, which by the definition of entropy numbers has cardinality $\card(K) = 2^{n-1}$. Since $m^b \geq 2^n > 2^{n-1}$, there must be $x \in K$ such that two distinct $y,z \in P^b$ are contained in the ball $x +  \delta B_{\ell_\infty^b(\ell_u^d)}$. Thus,
%\[ 
% \varepsilon < \|y - z\|_{\infty,u} \leq \|y - x\|_{\infty,u} + \|z-x\|_{\infty,u} \leq 2 \delta.
%\]
%This implies the left-hand side inequality.
%
%\textbf{Upper bound:} Let $m = 2^{\lfloor (n-1)/b + 1 \rfloor-1}$ and $\varepsilon = e_{\lfloor (n-1)/b+1 \rfloor}(\id: \ell_q^d \to \ell_u^d)$. Consider a minimal $\varepsilon$-covering of $B_{\ell_q^d}$ in $\ell_u^d$, which we denote by $K$. By the definition of entropy numbers, we have $\card(K) = m$. The Cartesian product $K^b$ is an $\varepsilon$-covering of $B_{\ell_\infty^b(\ell_q^d)}$ in $\ell_\infty^b(\ell_u^d)$ with cardinality $m^b$. The right-hand side inequality now follows since $m^b \leq 2^{n-1}$.
%\end{proof}

\subsection{Packing constructions}

\begin{lemma}\label{lem:general_packing}
Let $X,Y$ be (quasi-)Banach spaces and $\alpha_Y$ the quasi-norm constant of $\|\cdot\|_Y$. Let $0<p,r \leq \infty$, and $b \in \N$ with $b \geq 8$. For every $s \in [ \lfloor b/8 \rfloor ]$ and every $\varepsilon > 0$, there is a set of $2s$-block sparse elements $W \subseteq B_{\ell_p^b(X)}$ such that
\[ 
 \mathcal P\big(W, \|\cdot\|_{\ell_r^b(Y)}, s^{1/r-1/p} \varepsilon/(2^{1+1/p}\alpha_Y)\big) \geq \left(\frac{b \mathcal P(B_X, \|\cdot\|_Y, \varepsilon)}{32s}\right)^s.
\]
\end{lemma}
\begin{proof}
Let $W_0$ be a maximal $\varepsilon$-packing of $B_X$ in $Y$, i.e., $ m := \card(W_0) = \mathcal P(B_X, \|\cdot\|_Y, \varepsilon)$. Note that for each $x \in W_0$, we have $\|x\|_Y \geq \varepsilon/(2\alpha_Y)$. According to Lemma \ref{lem:Gilbert}, there is a subset $\widetilde{W}_s$ of the $2s$-fold Cartesian product $W_0^{2s}$ with cardinality
\[ 
 \card(\widetilde{W}_s) \geq \frac{m^{2s}}{\sum_{k=0}^{s-1} {2s \choose k} (m-1)^k} \geq \frac{m^{2s}}{2^{2s} m^s} = m^s /4^s,
\]
such that $\|x-y\|_{\ell_r^{2s}(Y)} \geq s^{1/r}\varepsilon$ for any two distinct $x,y \in \widetilde{W}_s$.

Next, we construct a suitable set of $2s$-block sparse elements in $B_{\ell_p^b(X)}$ based on $\widetilde{W}_s$. Using Lemma~\ref{lem:subsets}, we pick a sequence $(I_{\al})$ of $(b/(8s))^s$ subsets of $[b]$ such that each $I_{\al}$ has cardinality $2s$ and
$$\card(I_{\al} \cap I_{\ga}) < s \ \ \text{ whenever } \al \neq \ga.$$
Consider the set of $2s$-block sparse elements
\[ 
 W = \bigcup_{\alpha}  \left\lbrace x = (2s)^{-1/p} (x_1,\dots,x_b) \in \ell_p^b(X): x_{I_\alpha} \in \widetilde{W}_s, x_{[b] \setminus I_\alpha} = 0 \right\rbrace \subset B_{\ell_p^b(X)}.
\]
This set has cardinality $(b/(8s))^s \card(\widetilde{W}_s)$. Consider any $x,y \in W$ with $x \neq y$ and support sets $I_\alpha, I_\gamma$. We have to distinguish to cases to estimate the $\ell_r^b(Y)$-distance. If $I_\alpha = I_\gamma$, then
\[ 
 \|x-y\|_{\ell_r^b(Y)} \geq 2^{-1/p} s^{1/r-1/p} \varepsilon.
\]
If $I_\alpha \neq I_\gamma$, then
\[ 
 \|x-y\|_{\ell^b_r(Y)} = \Big( \sum_{i \in I_\alpha \cap I_\gamma} \|x_i - y_i\|_Y^r +  \sum_{i \in (I_\alpha \setminus I_\gamma) \cup (I_\gamma \setminus I_\alpha)}  \|x_i - y_i\|_Y^r \Big)^{1/r} \geq \frac{(2s)^{1/r-1/p} \varepsilon}{2\alpha_Y}.
\]
With the usual modification in case that $r=\infty$, the result follows.
\end{proof}

\begin{corollary}
\label{lem:sparsePacking}
Let $b,d \in \N$ with $b,d \geq 8$. For any $0<p,q,r,u\leq \infty$, $s \in [\lfloor b/8\rfloor]$, and $t \in [\lfloor d/8 \rfloor]$, there is a set $W$ of $(2s,2t)$-sparse vectors in $B_{\mixedell{p}{q}}$ such that
$$\cP(W,\|\cdot\|_{\ell_r^b(\ell_u^d)},s^{1/r-1/p} t^{1/u-1/q})\geq \Big(\frac{b}{32s}\Big)^s\Big(\frac{d}{8t}\Big)^{st}.$$
\end{corollary}
%\begin{proof}
%For every $k\in [b]$, use Lemma~\ref{lem:subsets} to find a sequence $(J_{\beta}^{(k)})_{\beta}$ of $(d/(8 t))^{t}$ subsets of $[d]$ such that each $J_{\beta}^{(k)}$ has cardinality $2t$ and
%$$\card(J_{\beta}^{(k)} \cap J_{\delta}^{(k)}) < t \ \ \text{ whenever } \beta \neq \delta.$$
%Next, using Lemma~\ref{lem:subsets} we pick a sequence $(I_{\al})$ of $(b/(8s))^s$ subsets of $[b]$ such that each $I_{\al}$ has cardinality $2s$ and
%$$\card(I_{\al} \cap I_{\ga}) < s \ \ \text{ whenever } \al \neq \ga.$$
%We now define $W$ to be the set of vectors
%$$x_{\al,\beta} = \sum_{i\in I_{\al}}\sum_{j\in J_{\beta}^{(i)}} e_{ij},$$
%where $e_{ij}$ are the standard basis vectors in $\R^{b\ti d}$. For every fixed $\al$ there are $(d/(8 t))^{st}$ different vectors $x_{\al,\beta}$ and therefore the cardinality of $W$ is $(b/(8s))^s(d/(8 t))^{st}$. Moreover,
%$$\|x_{\al,\beta}\|_{\ell_p^b(\ell_q^d)} = \Big(\sum_{i\in I_{\al}}\Big(\sum_{j\in J_{\beta}^{(i)}}\Big)^{p/q}\Big)^{1/q}\leq (2s)^{1/p}(2t)^{1/q}$$
%and
%\begin{align*}
%\|x_{\al,\beta} - x_{\ga,\del}\|_{\ell_p^b(\ell_q^d)} & = \Big(\sum_{i\in I_{\al}\cap I_{\ga}} \Big(\sum_{j\in J_{\beta}^{(i)}\Delta J_{\del}^{(i)}}\Big)^{p/q} + \sum_{i\in I_{\al}\setminus I_{\ga}} \Big(\sum_{j\in J_{\beta}^{(i)}}\Big)^{p/q} \\
%& \qquad \qquad + \sum_{i\in I_{\ga}\setminus I_{\al}} \Big(\sum_{j\in J_{\del}^{(i)}}\Big)^{p/q}\Big)^{1/p} \geq s^{1/p} (2t)^{1/q}.
%\end{align*}
%This completes the proof.
%\end{proof}

\begin{remark}
In case that $r=\infty$, we obtain a version of Lemma \ref{lem:general_packing} with better constants since we do not have to rely on the combinatorial Lemma \ref{lem:Gilbert} but use the full Cartesian product $W_0^{2s}$ instead. This leads to the bound
\[ 
 \mathcal P\big(W, \|\cdot\|_{\ell_\infty^b(Y)}, s^{1/r-1/p} \varepsilon/(2^{1+1/p}\alpha_Y)\big) \geq \left(\frac{b \mathcal P(B_X, \|\cdot\|_Y, \varepsilon)}{8s}\right)^s.
\]
\end{remark}

\subsection{Equal outer spaces}\label{sec:entropy:p=r}

We begin our considerations with the situation that the outer spaces coincide. That is, for $X, Y$ being (quasi-)Banach spaces, we consider the entropy numbers
\[ 
 e_n(B_{\ell_p^b(X)}, \ell_p^b(Y)).
\]

The generalized Edmunds-Triebel covering considered in Proposition \ref{res:generalization_Edmunds_Triebel} is optimal in case that $q=u$. This is a consequence of the following lower bound, which improves the general lower bound given in Lemma \ref{res:entropy_lb_volarg} for $n \leq nb$.

\begin{proposition}\label{res:equal_inner_spaces_lb}
Let $0< p < r \leq \infty$ and $0< q \leq \infty$. Further assume $d,b \geq 8$. Then,
\begin{align*}
e_n(\id: \ell_p^b(\ell_q^d) \to \ell_r^b(\ell_q^d)) \geq c_{p,r,q}
\begin{cases}
 1 &:\; 1 \leq n \leq d + \log_2(b)\\
 \left[\frac{\log(eb/n))+d}{n}\right]^{1/p - 1/r} &:\; d + \log_2(b) \leq n \leq bd\\
\end{cases}
\end{align*}
\end{proposition}

\begin{proof}
Recall Lemma \ref{lem:sparsePacking}, according to which there is a set $W$ of $(s,t)$-sparse vectors with cardinality $\card(W) \geq (b/(4s))^{s/2} (d/(4t))^{st/4}$ such that $W \subseteq B_{\mixedell{p}{q}}$ and
\[ 
 \|x - y\|_{\mixedell{r}{q}} \geq s^{1/r-1/p}.
\]
The proof's essence is to choose $s$ and $t$ suitably for given $n \in [bd]$ to obtain the lower bound. We give a concise formulation of the proof at this point, which omits technicalities. Tedious details can be found in Appendix \ref{detail:lb_equal_inner_spaces}, including rather precise formulae for the constants. We obtain the first lower bound,
\[ 
 e_n(\id: \ell_p^b(\ell_q^d) \to \ell_r^b(\ell_u^d)) \gtrsim 1
\]
for all $n \lesssim d + \log_2(b)$, if we choose $s\simeq 1$ and $t \simeq d$, i.e., the packing consists of $1$-outer sparse matrices with each non-vanishing row being dense (no inner sparsity).

For the second lower bound, we again vary only the outer sparsity $s$ according to the given $n \in [bd]$, namely
\[
 s \simeq \frac{n}{\log_2(eb/n)+d}
\]
such that $n-1 \leq s (\log_2(eb/s)+d) \lesssim \log_2(\card(W))$. This yields the lower bound
\[ 
 e_n(\id:\mixedell{p}{q} \to \mixedell{r}{q}) \geq 1/2 \, s^{1/r-1/p} \gtrsim \left( \frac{\log_2(eb/n)+d}{n}\right)^{1/p-1/r}
\]
for $d+ \log_2(b) \leq n \lesssim b2^{d/16}$. Hence, for small $d$, it remains to consider $bd \geq n \gtrsim b2^{d/16}$. Theorem \ref{res:entropy_lb_volarg} yields
\[ 
 e_n(\id:\mixedell{p}{q} \to \mixedell{r}{q}) \geq e_{bd+1}(\id:\mixedell{p}{q} \to \mixedell{r}{q}) \gtrsim b^{1/r-1/p} \gtrsim \big(\frac{d}{n-1}\big)^{1/p-1/r}.
\]
In the considered range, we can further estimate
\[ 
\big(\frac{d}{n-1}\big)^{1/p-1/r} \gtrsim \left(\frac{\log_2(eb/n)+d}{n}\right)^{1/p-1/r}.
\]
\end{proof}

\begin{remark}
We have polished not only the argumentation but also the lower bounds in Theorem \ref{res:equal_inner_spaces_lb} for reasons of clarity. The price are worse constants. Without polishing, the proof given in Appendix \ref{detail:lb_equal_inner_spaces} gives the following lower bound:
\begin{align*}
 e_n(\id: \mixedell{p}{q} \to \mixedell{r}{u}) \geq
 \begin{cases}
 (1/2)^{1/p-1/r+1} &: 0 \leq n-1 \leq \frac{d}{16} + \log_2(\frac{b}{8\sqrt{2}}),\\
 2^{1/p-1/r-1}\left[\frac{\log(\frac{b}{4\sqrt{2}(n-1)})+\frac{d}{16}}{n-1}\right]^{1/p - 1/r} &: \frac{d}{16} + \log_2(\frac{b}{8\sqrt{2}}) \leq n-1 \leq \frac{b2^{d/16}}{2^{2+e/2}},\\
 c_{p,q} \big(\frac{d}{n-1}\big)^{1/p-1/r} &: \frac{b2^{d/16}}{2^{2+e/2}} \leq n \leq bd.
 \end{cases}
\end{align*}
\end{remark}

\begin{remark}
In case that additionally $q < u$, the just presented proof yields the following lower bounds.
\begin{align*}
 e_n(\id: \mixedell{p}{q} \to \mixedell{r}{u}) \geq c_{p,q,r}
 \begin{cases}
 1 &: 1 \leq n \leq \log_2(bd),\\
 (1/d)^{1/q-1/u} &: \log_2(bd) \leq n \leq d + \log_2(b),\\
 (1/d)^{1/q-1/u} \left[\frac{\log(eb/n))+d}{n}\right]^{1/p - 1/r} &: d + \log_2(b) \leq n \leq bd.
 \end{cases}
\end{align*}
Note that the first lower bound follows trivially from the fact that there are $bd$ different matrices in $B_{\mixedell{p}{q}}$ which have only one non-vanishing entry and pairwise $\mixedell{r}{u}$-distance $1$.
\end{remark}

% % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % %

\subsection{Upper bounds and covering constructions}\label{sec:entropy:q=u}
Theorem \ref{thm:entropy_characterization_p} below shows that essentially the same relation as stated in Proposition \ref{thm:entropy_characterization_infty} holds true for $p < \infty$, as well (as one would expect). However, the suitable construction of a packing and a covering is much more involved as we cannot use simple $b$-fold Cartesian products anymore. The key idea of our proof is to pack respectively cover the ball $B_{\ell_p^b(X)}$ with a union of appropriately rescaled Cartesian products.
\begin{theorem}\label{thm:entropy_characterization_p}
Let $X,Y$ be (quasi-Banach) spaces and denote by $\alpha_Y$ the quasi-Banach constant of $Y$. Let $0<p \leq \infty$. Then, for $n \in \N$, we have
\[ 
 (\alpha_Y)^{-1} \, 2^{-1-1/p} \, e_{8n+1}(B_X,Y) \leq e_{nb}(B_{\ell_p^b(X)}, \ell_p^b(Y)) \leq 2^{1+1/\tilde p} e_{n-1}(B_X,Y),
\]
where $\tilde p = \min\{1,p\}$.
\end{theorem}

\begin{proof}
%We prove
%\[
% 2^{-1-1/p} \, e_{\lceil 2n/b+1 \rceil}(\id: \ell_q^d \to \ell_u^d) \leq e_n(\id: \ell_p^b(\ell_q^d) \to \ell_p^b(\ell_u^d)) \leq 2^{1+1/\tilde p} \, e_{\lfloor (n-1)/b \rfloor}(\id: \ell_q^d \to \ell_u^d),
%\]
%We just describe the specific covering and packing construction. For the rest the argumentation is standard and analogously to the case $p = \infty$.

\emph{Lower bound.} For $\varepsilon > 0$, let $x_1,\dots,x_m$ be a maximal $\varepsilon$-packing of $B_X$ in $Y$. Obviously, we have $\|x\|_Y \geq \varepsilon/(2\alpha_Y)$ for at least $m-1$ elements of $\mathcal P$, say $x_1,\dots,x_{m-1}$. According to Lemma \ref{lem:subsets}, there are $N \geq 2^{b/16}$ many subsets $I_1,\dots,I_N \subseteq [b]$ such that $\sharp I_k = b/8$ and $\sharp (I_k \cap I_j) < b/16$ whenever $k \neq j$. Now consider the set $\mathcal P$ given by
\[ 
 \mathcal P = \bigcup_{k=1}^N \{ x= (b/8)^{-1/p}(x_{1\cdot},\dots, x_{b\cdot}) \in \R^{bd}: x_{i\cdot} \in \{x_1,\dots, x_{m-1} \} \text{ if } i \in I_k, x_{i\cdot} = 0 \text { otherwise } \}.
\]
This set has cardinality $\sharp \mathcal P \geq 2^{b/16} (m-1)^{b/8}$ and for every $x \in \mathcal P$, $\|x\|_{\ell_p^b(X)} \leq 1$. Furthermore, for $x,y \in \mathcal P$ with $x \neq y$, we observe
\[ 
 \|x-y\|_{\ell_p^b(Y)} \geq 2^{-1/p-1} \varepsilon/\alpha_Y.
\]
It remains to do some standard calculations to obtain the lower bound.

\emph{Upper bound.} We use the following covering construction. For every $w \in B_{\ell_p^b}$, define the set 
\[ 
 B_w := \{ x \in B_{\ell_p^b(X)}: |\|x_{i\cdot}\|_X - w_i| \leq b^{-1/p} \text{ for } i \in [b] \}.
\]
Clearly, $B_w \subseteq \times_{i=1}^b (w_i + b^{-1/p})B_X =: U_w$. Let $w^1,\dots,w^{2^b}$ be a minimal $b^{-1/p}$-covering of $B_{\ell_p^b}$ in $\ell_\infty^b$. Then, we have
\[ 
 B_{\ell_p^b(X)} \subseteq \bigcup_{i=1}^{2^b} B_{w^i}.
\]
Now, let $\Gamma$ be a minimal $\varepsilon$-covering of $B_X$ in $Y$ with cardinality $m$. Consider the Cartesian product $\Gamma_w = \times_{i=1}^b (w_i + b^{-1/p})\varepsilon \Gamma$, which has cardinality $m^b$. For $x \in U_w$, there is $v \in \Gamma_w$ such that
\[ 
 \|x - v\|_{\ell_p^b(Y)} = \big(\sum_{i=1}^b \|x_{i\cdot} - v_{i\cdot}\|_Y^p \big)^{1/p} \leq \big( (w_i + b^{-1/p})^p \varepsilon^p \big)^{1/p} \leq 2^{1/\tilde p} (\|w\|_p + 1)\varepsilon \leq 2^{1+1/\tilde p} \varepsilon,
\]
where $\tilde p = \min\{1,p\}$. Hence the set $\bigcup_{i=1}^{2^b} \Gamma_{w^i}$ is a $2^{1+1/\tilde p} \varepsilon$-covering of $B_{\ell_p^b(X)}$ in $\ell_p^b(Y)$ with cardinality $2^b m^b$. Doing some standard calculations, we obtain the upper bound.
\end{proof}

\begin{remark}
The upper bound in Theorem \ref{thm:entropy_characterization_p} could also be proved based on a covering construction that has recently appeared in a work by Edmunds and Netrusov, see \cite[Lem. 2.2, Lem. 2.3, Lem 2.4]{EdNe2015}.
\end{remark}

\begin{remark}
We leave the setting of equal outer spaces to discuss a further, very general covering construction known in the literature. Let $X_1,\dots,X_b$ and $Y_1,\dots, Y_b$ be (quasi-)Banach spaces and $0<p,r\leq \infty$. The covering rests on the idea to split the ball $B_{\ell_p^b({X_1,\dots,X_b})}$ into subsets of matrices with non-increasing rows,
\[ 
B_{\ell_p^b({X_1,\dots,X_b})} \subseteq \bigcup_\pi \{ x \in B_{\ell_p^b({X_1,\dots,X_b})}: \|x_{\pi(1)\cdot}\|_{X_1} \geq \dots \geq \|x_{\pi(b)\cdot}\|_{X_b} \},
\]
where the union is taken over all permutations of $[b]$. To our knowledge, this construction appeared first in \cite[Proof of Prop. 4]{KLSS06} and leads to the upper bound
\begin{align}\label{eq:covering_KLSS} 
 e_{\sum_{j=1}^b n_j + b \log_2(b)}\big(B_{\ell_p(\{X_j\}_{j=1}^b)}, \ell_r(\{Y_j\}_{j=1}^b)\big) \leq \big( \sum_{j=1}^b j^{-r/p} e_{n_j}(B_{X_j}, Y_j)^r\big)^{1/r}
\end{align}
for $n_1,\dots,n_b \in \N$. We point out that \eqref{eq:covering_KLSS} in general does not allow to reproduce the upper bound in Theorem \ref{thm:entropy_characterization_p}. However, in case that $X=X_1=\dots=X_b=\ell_q^d$ and $Y=Y_1=\dots=Y_b=\ell_u^d$ with $0<q\leq u$, \eqref{eq:covering_KLSS} provides an alternative to Theorem \ref{thm:entropy_characterization_p} to obtain the upper bound in Theorem \ref{res:entropy_matching_bounds} (ii) below.
\end{remark}

The covering constructions presented in the previous chapter work well for parameter constellations where $1/q - 1/u > 1/p - 1/r$, i.e., the difference between the inner spaces dominates the difference between the outer spaces. For equal inner spaces ($q=u$), we need a different approach. It turns out that a generalization of the well-known Edmunds-Triebel covering \cite{EdTr96} yields matching upper bounds. The classical Edmunds-Triebel covering is used to for the entropy numbers $e_n(B_{\ell_p^b}, \ell_\infty^b)$, $0<p < \infty$, in the preasymptotic range $1 \leq n \leq b$. Its key idea is that, given any element $x$ in the $\ell_p^b$-unit ball, at most $k$ components of $x$ can be larger than $k^{-1/p}$, which is why a $k^{-1/p}$-covering of $B_{\ell_p^b}$ can be constructed from $k$-sparse vectors. We generalize this idea for mixed spaces by replacing $k$-sparse vectors by $k$-block sparse matrices. This yields the following upper bound.

%Let us first consider the situation in which the inner spaces coincide ($q=u$) and $p < r$, that is, relative to the error norm $\|\cdot\|_{\mixedell{r}{q}}$ we deal with block-compressible matrices. Recalling the well-known behavior of the entropy numbers $e_n(B_{\ell_q^d}, \ell_q^d)$, we expect the inner dimension $d$ to appear in main terms of the bounds while the specific value of $q$ should only affect the constants. In consequence, apart from the effect of the inner dimension $d$, we expect the entropy numbers $e_n(B_{\ell_p^b(\ell_q^d)}, \ell_r^b(\ell_q^d))$ to behave very much like the entropy numbers $e_n(B_{\ell_p^b}, \ell_r^b)$. Indeed, the following covering construction turns out to be optimal: in the same fashion as one would use sparse vectors to construct a covering of $B_{\ell_p^b}$ in $\ell_r^b$, we use block-sparse matrices to cover $B_{\mixedell{p}{q}}$ in $\mixedell{r}{q}$; see Subsection \ref{sec:entropy:q=u} for details. This leads to the following matching bounds.

\begin{proposition}[Generalization of Edmunds-Triebel-covering]\label{res:generalization_Edmunds_Triebel}
Let $0<p,q,r \leq \infty$ and $d>2$. Then, for $1 \leq n \leq bd$,
\begin{align*}
e_n(\id: \ell_p^b(\ell_q^d) \to \ell_r^b(\ell_q^d)) \leq C_{p,q,r}
 \left[\frac{\log(eb/n)+d}{n}\right]^{1/p - 1/r}.
\end{align*}
\end{proposition}

\begin{proof}
We first consider $p=\infty$ and describe the covering construction. Let $k \in [b]$. Since at most $k$ rows of any $x \in B_{\mixedell{p}{q}}$ can have a $q$-norm $\|x_{i \cdot}\|_q \geq k^{-1/p}$, it follows that
\[ 
 B_{\mixedell{p}{q}} \subseteq \bigcup_{I \subseteq [b]: |I| = k} B_I,
\]
where $ B_I := \{ x \in B_{\mixedell{p}{q}} : \|x_{i\cdot}\|_q \geq k^{-1/p} \text{ for } i \in I\}$.
According to Proposition \ref{res:entropy_ub_volarg} we have
\[ 
 e_{1+c_{p,q}kd}( \id: \ell_p^k(\ell_q^d) \to \ell_\infty^k(\ell_q^d) ) \leq C_{p,q} k^{-1/p}.
\]
Hence, for any $I \subseteq [b]$ with $|I| = k$, if we take a minimal $C_{p,q}k^{-1/p}$-covering of $B_{\ell_p^k(\ell_q^d)}$ in $\ell_\infty^k(\ell_q^d)$ and append $b-k$ zero rows to every matrix of the covering, then we obtain a $C_{p,q}k^{-1/p}$-covering of $B_I$ with cardinality $2^{c_{p,q}kd}$. Repeating this procedure for every possible index set yields a $C_{p,q}k^{-1/p}$-covering $\mathcal U$ of $B_{\mixedell{p}{q}}$ in $\mixedell{\infty}{q}$ with cardinality
\[
 \card(\mathcal U) = {b \choose k} 2^{c_{p,q}kd}.
\]

Now, given $n \in [bd]$, we choose $k \simeq \frac{n}{\log(eb/n)+d}$ such that $\log(\card(\mathcal U))  \lesssim k (\log(eb/k)+d) \leq n-1$ is assured. Consequently, we obtain the upper bound
\[ 
 e_n(\id: \mixedell{p}{q} \to \mixedell{\infty}{q}) \lesssim k^{-1/p} \lesssim \left(\frac{\log_2(eb/n)+d}{n}\right)^{1/p}.
\]
Note that we have omitted some technical details in the last two arguments. These can be found in Appendix \ref{detail:edmunds_triebel}, including a detailed account of constants.
Finally, we note that the case $r < \infty$ now follows by a standard interpolation argument, see \cite{EdTr96}.
\end{proof}

\begin{remark}
Basically the same generalization of the Edmunds-Triebel covering construction as in Proposition \ref{res:generalization_Edmunds_Triebel} is given in the recent work \cite{EdNe2015}. Concretely, for $T$ a general linear operator and $X$, $Y$ q-normed quasi-Banach spaces, \cite[Thm 3.1]{EdNe2015} provides matching bounds for the entropy numbers $e_n(T: \ell_p^b(X)  \to \ell_r^b(Y))$ in the range $ \log(b) \leq n \leq b$. Thus, the general theorem \cite[Thm 3.1]{EdNe2015} reproduces the specific matching bounds found in Theorem \ref{res:entropy_matching_bounds} (i) for $ \log(b) \leq n \leq b$, for larger $b < n \leq bd$ it does not apply.
\end{remark}

\section{Matching bounds for entropy numbers of $\ell_p(\ell_q)$-spaces}\label{sec:entropy_matching_bounds}

\noindent Subject of this section is to characterize the behavior of the entropy numbers
\[ 
 e_n(B_{\ell_p^b(\ell_q^d)}, \ell_r^b(\ell_u^d)), \qquad 0<p \leq r\leq \infty, 0< q \leq u \leq \infty,
\]
for all $n, b, d \in \N$. For large $n \geq bd$ and very small $n \leq \log(bd)$, it requires only very standard arguments to obtain matching bounds for all parameter constellations. For the sake of completeness, we write down the bounds, which should be no surprise for the reader familiar with entropy numbers.

\begin{proposition}\label{thm:entropy_characterization_infty}
Let $X,Y$ be (quasi-)Banach spaces. Then, for $n \in \N$, we have
\[ 
 \frac{e_{n+1}(B_X,Y)}{2} \leq e_{nb}(B_{\ell_\infty^b(X)}, \ell_\infty^b(Y)) \leq e_n(B_X,Y).
\]
\end{proposition}

\begin{proposition}\label{res:entropy_easy_cases} Let $0<p \leq r\leq \infty, 0< q \leq u \leq \infty$.
 \begin{align*} 
  e_n(B_{\ell_p^b(\ell_q^d)}, \ell_r^b(\ell_u^d)) \simeq
  \begin{cases}
    1 &: n \leq \log(bd),\\
    b^{1/r-1/p} d^{1/u-1/q} 2^{-\frac{n-1}{bd}} &: n \geq bd.
  \end{cases}
 \end{align*}
\end{proposition}
\begin{proof}
First note that  $e_n(B_{\ell_p^b(\ell_q^d)}, \ell_r^b(\ell_u^d)) \leq 1$ since $B_{\ell_p^b(\ell_q^d)} \subseteq B_{\ell_r^b(\ell_u^d)}$. For $n \leq \log(bd)$, 
the bounds now follow trivially from the fact that  there are $bd$ different matrices in the $\mixedell{p}{q}$-unit ball which have only one non-vanishing entry and pairwise $\mixedell{r}{u}$-distance $1$. The bounds for large $n$ follow by standard volumetric arguments, see Lemma \ref{res:entropy_lb_volarg} and Lemma \ref{res:entropy_ub_volarg} in the appendix.
\end{proof}

What we are really concerned with in this paper is the preasymptotic range $\log(bd) \leq n \leq bd$. Here, interesting and unexpected effects occur. In Theorem \ref{res:entropy_matching_bounds}, we summarize the parameter constellations where we obtain matching bounds. Surprisingly, in those constellations, the decay in $n$ is either determined by the relation of the outer spaces $1/p-1/r$ or the relation of the inner spaces $1/q-1/u$, but not by both at the same time. We point out that the first upper bound in Theorem \ref{res:entropy_matching_bounds} (iv) is due to \cite{Vyb06}.

\begin{theorem}\label{res:entropy_matching_bounds}
Let $0<p \leq r\leq \infty, 0< q \leq u \leq \infty$, and $n \in \N$. In the range $\log(bd) \leq n \leq bd$, we observe in dependence on the values of $p,q,r,u$ the following behavior of entropy numbers:
\begin{enumerate}[label=(\roman*)]
 \item If $q = u$ and $p < r$, then
    \begin{align*}
     e_n(B_{\ell_p^b(\ell_q^d)}, \ell_r^b(\ell_q^d)) \simeq
     \begin{cases}
      1 &: \log(bd) \leq n \leq d + \log_2(b),\\
      \left(\frac{\log_2(eb/n)+d}{n}\right)^{1/p-1/r} &: d+\log_2(b) \leq n \leq bd.
     \end{cases}
    \end{align*}
 \item If $p=r$ and $q\leq u$, then we have
 \begin{align*}
  e_n(B_{\ell_p^b(\ell_q^d)}, \ell_p^b(\ell_u^d)) \simeq
  \begin{cases}
   1 &: \log(bd) \leq n \leq b \log_2(d)\\
   \left(\frac{b \log_2(ebd/n)}{n}\right)^{1/q-1/u} &: b\log_2(d) \leq n \leq bd
  \end{cases}
 \end{align*}
 \item If $r=u$ and $0<q<p<r$, then we have
  \begin{align*}
   e_n(B_{\ell_p^b(\ell_q^d)}, \ell_r^b(\ell_r^d)) \simeq
   \begin{cases}
   \left(\frac{\log_2(ebd/n)}{n}\right)^{1/p-1/r} &: \log(bd) \leq n \leq b\log(d)\\
   b^{1/r-1/p} \left(\frac{b\log(ebd/n)}{n}\right)^{1/q-1/r} &: b\log(d) \leq n \leq bd\\
   \end{cases}
  \end{align*}
  \item If $1/q-1/u > 1/p - 1/r > 0$, then
  \[ 
   e_n(B_{\ell_p^b(\ell_q^d)}, \ell_r^b(\ell_u^d)) \simeq  b^{1/r-1/p} \left(\frac{b\log(ebd/n)}{n}\right)^{1/q-1/u}
  \]
  for $b\max\{\log(d),\log(b)\} \leq n \leq bd$. If we additionally assume $q < p < r < u$ and $b \leq d$, then
  \[ 
      e_n(B_{\ell_p^b(\ell_q^d)}, \ell_r^b(\ell_u^d)) \simeq
      \begin{cases}
      \left(\frac{\log_2(ebd/n)}{n}\right)^{1/p-1/r} &: \log(bd) \leq n \leq b\log(d)\\
      b^{1/r-1/p} \left(\frac{b\log(ebd/n)}{n}\right)^{1/q-1/u} &: b\log(d) \leq n \leq bd\\
      \end{cases}
  \]
\end{enumerate}
\end{theorem}

\begin{proof}
\emph{Ad (i).}
The upper bound follows from a generalization of the well-known Edmunds-Triebel covering construction to block-sparse matrices, see Proposition \ref{res:generalization_Edmunds_Triebel}. For the lower bound, see Proposition \ref{thm:equal_inner_spaces_lb}.

\emph{Ad (ii).}
According to Theorem \ref{thm:entropy_characterization_p}, we have for $n \in \N$ a multiple of $b$,
\[ 
 e_{2n/b+1}(B_{\ell_q^d},\ell_u^d) \lesssim_p e_n(B_{\ell_p^b(\ell_q^d),\ell_p^b(\ell_u^d)}) \lesssim e_{n/b-1}(B_{\ell_q^d},\ell_u^d).
\]
Hence, for $n$ a multiple of $b$, the statement follows from the well-known fact
\[ 
 e_k(B_{\ell_q^d},\ell_u^d) \simeq \left(\frac{\log(ed/k)}{k}\right)^{1/q-1/u}, \quad 1 \leq k \leq d.
\]
For arbitrary $1 \leq n \leq bd$, we obtain the result by monotonicity arguments.

\emph{Ad (iii).} First consider $\log(bd) \leq n \leq b\log(d)$. The lower bound can be derived using a packing argument: in Lemma \ref{lem:sparsePacking}, choose the inner sparsity $t$ constant, say $t=1$, and maximize the outer sparsity $s$. This gives a $(2s)^{1/r-1/p}$-packing of cardinality $\simeq (bd/s)^s$; see Appendix \ref{appendix} for details how to translate this into the desired lower bound for entropy numbers. The upper bound follows immediately from the inclusion $B_{\mixedell{p}{q}} \subset B_{\mixedell{p}{p}}$ and the classical result
\[ 
 e_n(\id: \ell_p^{bd} \to \ell_r^{bd}) \simeq_{p,r} \left(\frac{\log(ebd/n)}{n}\right)^{1/p-1/r}.
\]

Let us now consider $b\log(d) \leq n \leq  bd$. Observe that $B_{\mixedell{r}{q}} \subset b^{1/p-1/r} B_{\mixedell{p}{q}}$ and $B_{\mixedell{p}{q}} \subset b^{1/q-1/p} B_{\mixedell{q}{q}}$, simply by H\"older's inequality. Statement (i) then implies
\begin{align*}
 b^{1/r - 1/p} \left(\frac{b\log(ebd/n)}{n}\right)^{1/q-1/r}
 &\simeq_{q} b^{1/r -1/p} e_n(\id: \mixedell{r}{q} \to \mixedell{r}{r})\\
 &\leq e_n(\id: \mixedell{p}{q} \to \mixedell{r}{r})\\
 &\leq b^{1/q-1/p} e_n(\id: \mixedell{q}{q} \to \mixedell{r}{r})\\
 &\simeq_{q} b^{1/q-1/p} \left(\frac{\log(ebd/n)}{n}\right)^{1/q-1/r}
\end{align*}

\emph{Ad (iv).} The upper bound has already been proved in \cite[Lem. 3.16]{Vyb06}. We just note that the upper bound follows by Lemma 4.7 and the well-known behavior of $e_n(B_{\ell_q^d},\ell_u^d)$ if we choose $n_j \simeq j^{-\alpha}$ for some $0<\alpha<1$ such that $\alpha(1/q-1/u) > 1/p - 1/r$.
\end{proof}

\begin{remark}
The bounds in Theorem \ref{res:entropy_matching_bounds} (iii) suggest that the following covering construction is optimal. For small $n \leq b\log(d)$ we use only matrices in the covering which have at most one non-zero entry per row and optimize the number of non-zero rows. For $n > b \log(d)$ we do not exploit the block-compressibility anymore and instead rely solely on the stronger compressibility within blocks $q$ by optimizing the number of non-zero entries per row.
\end{remark}

==> todonote.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Auxiliary stuff for the working draft
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\usepackage{ifdraft}
% option colorinlistoftodos
\usepackage[linecolor=red,bordercolor=white, backgroundcolor=white,textsize=small,textwidth=3cm]{todonotes}
\usepackage{xcolor}
\usepackage{setspace}
\usepackage[normalem]{ulem}
\usepackage{comment}
\usepackage{framed}

\ifdraft{\usepackage{refcheck}}{}
%\ifdraft{\usepackage{showkeys}}{}

% TODO environment for comments in the text
% (for the spacing command the package setspace is required)
\newcounter{todocounter}
\newenvironment{todobox}[3][]
{\noindent\addtocounter{todocounter}{1}\todo[caption={\protect\hypertarget{todo\thetodocounter}{}#2 #3},noline, #1]{\hyperlink{todo\thetodocounter}{\textcolor{red}{#2 \thetodocounter}}}}
{}

% usage: \todonote[short text]{text}
\newcommand{\TODO}[2][]{\ifdraft{\begin{todobox}{TODO}{#1} \textcolor{red}{#2} \end{todobox}}{}}

%usage: \fix[title]{text}
\newcommand{\fix}[2][]{\ifdraft{\begin{todobox}{\textcolor{red}{FIXME}}{\textcolor{red}{#1}} \textcolor{red}{#2} \end{todobox}}{}}

%usage: \note[receiver]{text}
\newcommand{\note}[3][all]{\ifdraft{\hrule\vspace*{6pt}\begin{todobox}[noline,backgroundcolor=white,bordercolor=white]{@ #1}{#2} #3 \end{todobox}\vspace*{6pt}\hrule\vspace*{6pt}}{}}

\specialcomment{help}
{
\section*{Help}
}
{}
\ifdraft{}{\excludecomment{help}}

\specialcomment{changes}
{
\section*{Changes}
}
{\listoftodos[TODO's and Comments]}
\ifdraft{}{\excludecomment{changes}}

\specialcomment{detail}
{\vspace*{6pt}\hrule\vspace*{6pt}\marginpar{\small DETAIL}}
{\vspace*{6pt}\hrule\vspace*{6pt}}
\ifdraft{}{\excludecomment{detail}}

\newcommand{\old}[1]{\textcolor{red}{\sout{\ifdraft{#1}{}}}}
\newcommand{\new}[1]{\ifdraft{\textcolor{green!50!black}{#1}}{#1}}

%\begin{help}
%
%\begin{itemize}
% \item \new{Piece of text which is new in this version.}
% \item \old{Piece of text that should be removed for some reason.}
% \item \textcolor{blue!50!black}{/** more detailed descriptions; internal comments; $\dots$ **/}
% \item Remove the \texttt{draft} option to hide working draft annotations.
%\end{itemize}
%
%\end{help}
